Pipeflow: An Efficient Task-Parallel Pipeline Programming Framework using Modern C++

Pipeline is a fundamental parallel programming pattern. Mainstream pipeline programming frameworks count on data abstractions to perform pipeline scheduling. This design is convenient for data-centric pipeline applications but inefficient for algorithms that only exploit task parallelism in pipeline. As a result, we introduce a new task-parallel pipeline programming framework called Pipeflow. Pipeflow does not design yet another data abstraction but focuses on the pipeline scheduling itself, enabling more efficient implementation of task-parallel pipeline algorithms than existing frameworks. We have evaluated Pipeflow on both micro-benchmarks and real-world applications. As an example, Pipeflow outperforms oneTBB 24% and 10% faster in a VLSI placement and a timing analysis workloads that adopt pipeline parallelism to speed up runtimes, respectively.

==> Fig/micro_benchmark/throughput.tex <==
\begin{figure}[!h]
  \centering
  \pgfplotsset{
    title style={font=\LARGE},
    label style={font=\LARGE},
    %ylabel style={rotate=-90},
  }
  \begin{tikzpicture}[scale=0.49]
    \begin{axis}[
      title=Corun,
      %ymode=log,
      %xmode=log,
      %log basis x={2},
      ylabel=Throughput,
      xlabel=Number of Coruns,
      legend pos=north east,
    ]
    \addplot+ table[x=corun,y=tf,col sep=space]{Fig/micro_benchmark/throughput.txt};
    \addplot+ table[x=corun,y=tbb,col sep=space]{Fig/micro_benchmark/throughput.txt};
    \legend{Pipeflow, oneTBB}
    \end{axis}
  \end{tikzpicture}
  \caption{Throughput of corunning micro-benchmark worklaod.
  On the left, the pipeline structure consists of 80 serial stages and 80 parallel lines.
  On the right, the pipeline structure consists of 8 serial stages and 8 parallel lines. 
  Both run with 40 threads on 65K scheduling tokens.}
  \label{fig::micro-benchmark-throughput}
\end{figure}

